Hierarchical principles of embodied reinforcement learning: A review

Cognitive Psychology and related disciplines have identified several critical mechanisms that enable intelligent biological agents to learn to solve complex problems. There exists pressing evidence that the cognitive mechanisms that enable problem-solving skills in these species build on hierarchical mental representations. Among the most promising computational approaches to provide comparable learning-based problem-solving abilities for artificial agents and robots is hierarchical reinforcement learning. However, so far the existing computational approaches have not been able to equip artificial agents with problem-solving abilities that are comparable to intelligent animals, including human and non-human primates, crows, or octopuses. Here, we first survey the literature in Cognitive Psychology, and related disciplines, and find that many important mental mechanisms involve compositional abstraction, curiosity, and forward models. We then relate these insights with contemporary hierarchical reinforcement learning methods, and identify the key machine intelligence approaches that realise these mechanisms. As our main result, we show that all important cognitive mechanisms have been implemented independently in isolated computational architectures, and there is simply a lack of approaches that integrate them appropriately. We expect our results to guide the development of more sophisticated cognitively inspired hierarchical methods, so that future artificial agents achieve a problem-solving performance on the level of intelligent animals.

==> notes_snippets_manfred.tex <==

% This implies that different intelligent species would conceptualize the world in different ways, ultimately leading to different languages and different self-representations. 
% The theory states that there exist so-called basic concepts that are directly linked to the body. 
% As an example for a basic concept, consider the concept \concept{front}, which is determined by the direction in which we usually move and where most sensory organs are directed to. 
% Other more abstract concepts are hierarchically grounded in basic concepts. 
% For example, consider abstract mathematical concepts, where the front determines the geometric angle of $0^{\circ}$.

\citet{Shapiro2019_EmbodiedCognition} takes a weaker perspective, stating that also agents with different bodies can have shared mental concepts. The grounding of the concepts, however, may be different. He states that even an imaginative spherical being that is capable of omnidirectional movement and sensing in a gravitation-free environment can have a concept for \concept{front} if other objects or agents in its environment have a distinctive side that has certain front-typical features, such as eyes. However, for the spherical being, the \concept{front} concept is not a basic one because it is not directly linked to its body schema. 

Hence, the body schema has a strong influence on higher cognitive functions because it directly influences how we think. 
This becomes evident in natural language, where metaphorical expression involve basic body-related concepts \cite{Eppe2016_GCAI_SemanticParsing,Trott2016}. 
As an example, consider the metaphor \concept{up} \emph{is} \concept{more}. An agent that lives in a gravitation-free environment would not be able to understand a sentence like ``The stock market goes up''.


As an additional example of how body schemas influence our high-level cognitive operations consider recent work on \emph{concept blending} \cite{Eppe2018_AIJ_Blending,Confalonieri2016b,Confalonieri2015}. One pillar of human creativity is the capability of inventing new concepts by means of a serendipitous combinations of known concepts \cite{Fauconnier2002}. This concept blending process strongly depends on body-driven conceptualizations of the world. We conclude that, therefore, creative thought is also a result of the active self. 

What remains open, though, is how we can model grounding of sensorimotor concepts computationally. Several approaches,  including the Theory of Event-Coding \cite{Hommel2015_TEC}, and Event Segmentation Theory \cite{Zacks2007EventPerspective,Gumbsch2019AutonomousPrimitives}, exist. However it is subject to future work to fully integrate these approaches within a unifying computational theory of high-level cognition. Research on the minimal active self fosters the development of such a unifying theory because it allows one to investigate how basic body-related concepts emerge from sensorimotor interaction. 


\subsection{Representational state abstraction}
Cognitive scientists often model abstract mental concepts, such as \emph{path} of \emph{container} in terms of role-filler-based embodied semantic representations, such as semantic frames \cite{Barsalou1992} or image schemas \cite{Lakoff1988,Feldman2009_neural_ECG}. 
For example, a \concept{path} schema has a role \concept{trajector} which is typically filled by an object or agent that moves along the path, and it has roles for \concept{start} and \concept{end}. In our previous work on human-robot dialog, we build on image schemas to perform semantic parsing \cite{Eppe2016_IROS_SemanticParsing,Eppe2016_GCAI_SemanticParsing}, and show how embodied action-related representations facilitate semantic compositionality for human-robot interaction. 

Role-filler based representations are compatible with action-related semantic representations used in Artificial Intelligence. For example, in action planning, actions are commonly represented by sets of pre- and postconditions (cf. our previous work on action theory \cite{Eppe2015_JAL,Eppe2015_JAL_ASP}): a \concept{move-object} action has the precondition that the agent that moves the object must hold the object, and it has the postcondition that the object is at the target location. In our previous work \cite{Eppe2016_IROS_SemanticParsing,Eppe2016_GCAI_SemanticParsing}, we have used semantic action templates that link this pre- and postcondition perspective with the role-filler semantics of a semantic language parsing process. 
For example, the \concept{move-object} action inherits structure from the compositional \concept{path} concept: the object to move fills the \concept{trajector} role of the concept, the current object location fills that \concept{start} role and the target location fills the \concept{end} role. 

% , the current object location fills that \concept{start} role, and the target location the \concept{end} role. 

The Neurocognitive and Psychological theories of event coding \cite{Hommel2015_TEC} and ideomotor theory \cite{Stock2004} are in-line with the AI-based pre- and postcondition perspective on actions, as they consider associations between actions and effects at their core. 
However, these and other related theories do not provide a clear consensus on whether conceptual mental action representations are symbolic \cite{Barsalou1999} or distributed \cite{Hommel2015_TEC}. A unifying proposal of modern theories (e.g.~\cite{Hommel2010}) suggests that conceptual compositional representations are distributed, and that language serves as a symbolification mechanism for the underlaying distributed representations. 
\emph{However, there exists no commonly agreed upon mathematical model of learning compositional action- and state representations that is mechanistically compatible to the neurocognitive perspective of distributed representations that are potentially symbolifiable.} 


Humans abstract their sensorimotor data streams and map them to conceptual embodied representations \citet{Barsalou2008_GroundedCognition}. 
High-level cognitive representations and functions are algorithmically useful to arrange continuous low-level representations and functions into discrete representational spaces that are significantly smaller than continuous sensorimotor spaces. 
For example, on the lowest motor level, an \concept{open hand} action can be modelled as a sequence of continuous finger movements. The opening of the hand may be a semantic primitive within a high-level \concept{grasp} action that consists of \concept{[open hand, move hand to object, close hand]}. The grasp action itself may be a semantic primitive within another higher-level \concept{transport} behavior that consists of \concept{[grasp, move, release]}. 

This divide and conquer approach is also a prominent method to realize learning-based intelligent problem-solving behavior of robots and virtual agents. 

High-level cognitive representations and functions are algorithmically useful to arrange continuous low-level representations and functions into discrete representational spaces that are significantly smaller than continuous sensorimotor spaces. 
This effectively reduces the branching factor of a problem-solving search process: for the high-level action selection, an agent only has to consider a small set of discrete high-level action primitives and not the large set of their possible low motor-level instantiations. 
This computational problem-solving perspective on sensorimotor abstraction is in-line with



% This article is targeted at researchers in Artificial Intelligence and related fields. Therefore, we can impossibly cover all findings from the life sciences and human sciences that are related to problem-solving, decision-making and mental representations. But how can we obtain an objective overview about the state of the art on learning-based decision-making and problem-solving in cognitive psychology and cognitive neuroscience? 

% In this section, we address this question by performing a meta review of recent survey articles in cognitive psychology and animal cognition. We select and analyze the most cited review articles on learning-based problem-solving from the last three years, which we identify as follows:

% \begin{enumerate}
%     \item 
% \end{enumerate}

% The analysis reveals that there exist several theories related to representational abstraction and predictive forward models for learning-based problem-solving that are largely agreed upon and described well enough to be formalized within a computational framework. 
